Deep Spectral Clustering via Joint Spectral Embedding and Kmeans

Spectral clustering is a popular clustering method. It first maps data into the spectral embedding space and then uses Kmeans to find clusters. However, the two decoupled steps prohibit joint optimization for the optimal solution. In addition, it needs to construct the similarity graph for samples, which suffers from the curse of dimensionality when the data are high-dimensional. To address these two challenges, we introduce \textbf{D}eep \textbf{S}pectral \textbf{C}lustering (\textbf{DSC}), which consists of two main modules: the spectral embedding module and the greedy Kmeans module. The former module learns to efficiently embed raw samples into the spectral embedding space using deep neural networks and power iteration. The latter module improves the cluster structures of Kmeans on the learned spectral embeddings by a greedy optimization strategy, which iteratively reveals the direction of the worst cluster structures and optimizes embeddings in this direction. To jointly optimize spectral embeddings and clustering, we seamlessly integrate the two modules and optimize them in an end-to-end manner. Experimental results on seven real-world datasets demonstrate that DSC achieves state-of-the-art clustering performance.

==> sec_abstract.tex <==
Spectral clustering is a popular clustering method. It first projects data into the spectral embedding space and then uses Kmeans to find clusters. However, the two decoupled steps prohibit simultaneous optimization for the optimal solution. In addition, it needs to construct the similarity graph for data points, which suffers from the curse of dimensionality when the data are high-dimensional. To address these two challenges, we introduce \textbf{D}eep \textbf{S}pectral \textbf{C}lustering (\textbf{DSC}), which consists of the two main modules: the spectral embedding module and the entropy minimization module. The former module learns to embed raw data points into a discriminative low-dimensional spectral embedding space, which is spanned by the linear combinations of the top $k$ minimum eigenvectors of the graph Laplacian matrix. The latter module improves the cluster structures of Kmeans on the learned spectral embeddings by a greedy entropy-minimization strategy, which reveals the direction of the worst cluster structures and only optimizes in this direction. To simultaneously optimize spectral embeddings and clustering, we seamlessly integrate the losses of the two modules into a single joint loss. Experimental results on the real-world datasets demonstrate that DSC achieves state-of-the-art performance.
